Z Prime: A Story

This is an imaginary story that could come to pass involving a detector, a Boson, and good resolution. It was written for Snowmass 2013, as a white paper for the New Physics group. The story describes a scenario in which nature has designated the existence of a Left-Right Symmetric Model Z' at a pole mass of 3 TeV, which is observed by analysers through the dilepton decay channel. Signal and Background samples were generated for a proton-proton collider at $\sqrt{s}$ = 14 TeV and $\sqrt{s}$ = 33 TeV, with enough events to represent a dataset of up to 3000 fb$^{-1}$ for each centre of mass energy. These samples were passed through the Delphes fast simulation framework to produce detector reconstructed events. The story is played out from first hints to a well established new discovery with plentiful data, and attempts to capture the journey and excitement that this entails.

==> Magnetism/authorlist.tex <==
% list of HSPAW authors

%\hyphenpenalty 10000

\begin{center}

\begin{large} {\bf Conveners: D. Reggiano, R. Amati} \end{large}

A.~Alexandra, 
B. Bernitz, 
C. Claudsen, 
D. Duramucci, 
E. Ellifsen,
F. Forschungs, 
G. Gabriotti, 
H. Hudson, 
I. Izekevich, 
J. J. Jensen

\end{center}

%\hyphenpenalty 1000


==> Magnetism/wgreport.tex <==
%%%%%% Magnetism Chapter  %%%%%%%%%%%%%%%%
 
\chapter{Magnetic Influence on Cyanide Reagents}
\label{chap:mag}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{center}\begin{boldmath}

\input Magnetism/authorlist.tex
%Conveners are also listed separately in authorlist.tex

\end{boldmath}\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Introduction}
\label{sec:mag-intro}

Recently, F.  A. Mesmer \index{Mesmer}
has reported evidence of a profound influence of 
magnets on a variety of aspects of human and animal physiology~\cite{Mesmer}.
Numerous authors have claimed to reproduce certain of the phenomena 
reported by Mesmer~\cite{diCenzo,Muller}, but there is little understanding
of the precise mode of action of the magnetic influence.  In this
article, I will present evidence that mesmeric influence can disrupt the
lethal action of sodium cyanide (NaCN) when modulated by a sequence of 
high-pitched tones.  After a description of the phenomenon, I will comment
on the implications for the nature of the magnetic coupling.

\section{Observations}
\label{sec:mag-obs}

My observations began when I was called on an emergency basis to aid two
Albanian noblemen, Guglielmo B. and Ferrando di N., who had
ingested the poison in an apparent attempt to commit suicide.  (The facts
of the case were rather mysterious, since these young men had been seen in the 
harbor earlier in the day, affecting a carefree attitude.  However, this 
need not concern us here.)  The standard remedy would have been to induce
vomiting; however, this would have offended the 
sensibilities \index{sensibilities}  of two 
noble ladies present, the daughters of the duke in whose household this 
unfortunate incident took place.  Thus, I thought it wise to begin by 
administering magneto-therapy using the devices that I had at hand.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   use this format to include an .pdf figure into your paper
%%
\begin{figure}[htb]
\begin{center}
\includegraphics[width=0.3\hsize]{Magnetism/magnet.pdf}
\caption{Plan of the magnet used in the Mesmeric studies.}
\label{fig:magnet}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The source of magnetic influence used in this therapy was the simple
iron pole magnet shown in Figure~\ref{fig:magnet}.  The device, roughly
the size of human palm, was held three fingers' length away from each
of the patients, while the blood cyanide level was monitored.  As this 
operation proceeded in silence, only a very small effect on the poison was
observed.  In a moment, however, the sisters began to weep and ululate
in the most painful manner.  Under this blanket of sound, the effects of 
the cyanide reaction were observed to be completely reversed.  Indeed,
even before the end of a single session of treatment, the Albanians were
seen to wake from their comas and offer thanks for their rescue.  Some
sample blood cyanide levels are reported in Table~\ref{tab:blood}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%   use this format to include a LaTeX table  into your paper
%%
\begin{table}[t]
\begin{center}
\begin{tabular}{l|ccc}  
Patient &  Initial level($\mu$g/cc) &  w. Magnet &  
w. Magnet and Sound \\ \hline
 Guglielmo B.  &   0.12     &     0.10      &     0.001  \\
 Ferrando di N. &  0.15     &     0.11      &  $< 0.0005$ \\ \hline
\end{tabular}
\caption{Blood cyanide levels for the two patients.}
\label{tab:blood}
\end{center}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Interpretation}
\label{sec:mag-interp}

A description of these observations, obviously based on second-hand reports,
has already been reported by L. da Ponte~\cite{daPonte}. \index{da Ponte}
 In his paper,
da Ponte attributes the mode of action of the magnetic force to direct
magnetic attraction.  This would be implausible with the relatively small
magnet used in this study; thus da Ponte was forced to propose an absurdly
large size for the  magnetic device.  His theory does not account for the
acoustic influence, which is known not to be present in magnetic action on
inanimate objects.  A second hypothesis would state that the acoustic
fields perturb the chemistry of the cyanide reactions, allowing the 
reagents to couple magnetically.   As with the first hypothesis, we are
skeptical, since again this phenomenon has no inorganic counterpart.  Thus,
we are forced to conclude, with Mesmer, that magnetism couples directly to 
the life force, which, as is well known, can be modulated by musical 
influences.

In conclusion, we note that the unusual mode of action of magnetism is only
one of many which have been reported in the literature.  It is likely
that there are further unusual magnetic phenomena to be discovered.  All
studies to date have involved male patients.  But it is likely that the 
prevailing belief that `women are all the same' would be overturned in a
similar investigation.

NOTE ADDED:  Some more contemporary references on this topic can be 
found in \cite{Gansicke:2002zd,Barashenkov:2006ura,Ballarino:2010wva,Sheminova:2012cla}.

\Acknowledgements
I am grateful to Don Alfonso d'Alba for certain services essential to 
this investigation.  This work was supported by the US Department of Energy
     under contract DE--AC02--76SF00515.




\begin{thebibliography}{99}

%%
%%  bibliographic items can be constructed using the LaTeX format in SPIRES:
%%    see    http://www.slac.stanford.edu/spires/hep/latex.html
%%  SPIRES will also supply the CITATION line information; please include it.
%%

\bibitem{Mesmer}
F. A. Mesmer, Proc. Wien. Acad. Sci. {\bf 13}, 1564, 1593 (1762).
%%CITATION = PWASA,13,1564;%%

\bibitem{diCenzo}
A. L. di Cenzo, Trans. Acad. Ducal.  Milan., {\bf 23}, 2647 (1771).
%%CITATION = TAADD,23,2647;%%

\bibitem{Muller}
For an exhaustive review of the Prussian literature, see A. D. M\"uller,
in Workshop on Action at a Distance, F. Eisenschmidt, ed. (Springer,
Berlin, 1774).

\bibitem{daPonte}

L. da Ponte, Trans. N. Y. Acad. Sci., {\bf 3}, 27 (1795).
%%CITATION = TNYAA,3,27;%%



%\cite{Gansicke:2002zd}
\bibitem{Gansicke:2002zd} 
  B.~T.~Gansicke, F.~Euchner and S.~Jordan,
  %``Magnetic white dwarfs in the SDSS,''
  NATO Sci.\ Ser.\ II {\bf 105}, 199 (2003).
  %%CITATION = NSSIC,105,199;%%


%\cite{Barashenkov:2006ura}
\bibitem{Barashenkov:2006ura} 
  V.~S.~Barashenkov and H.~J.~Kaiser,
  %``Electric and Magnetic Polarizabilities of the Nucleons and Pions,''
  Fortsch.\ Phys.\  {\bf 10}, no. 2, 33 (1962).
  %%CITATION = FPYKA,10,33;%%
  %7 citations counted in INSPIRE as of 08 May 2013

%\cite{Ballarino:2010wva}
\bibitem{Ballarino:2010wva} 
  A.~Ballarino,
  %``Design of an MgB$_2$ feeder system to connect groups of superconducting magnets to remote power converters,''
  J.\ Phys.\ Conf.\ Ser.\  {\bf 234}, 032003 (2010).
  %%CITATION = 00462,234,032003;%%

%\cite{Sheminova:2012cla}
\bibitem{Sheminova:2012cla} 
  V.~A.~Sheminova,
  %``Investigation of the magnetic and temperature sensitivity of the Stokes parameters of absorption lines in the solar photosphere,''
  Kinematika i Fizika Nebesnych Tel {\bf 11}, 19 (1995)
  [arXiv:1211.2599 [astro-ph.SR]].
  %%CITATION = ARXIV:1211.2599;%%

\end{thebibliography}


\end{document}


==> tcilcomm.tex <==
% Macros used for TCI styles released with Scientific Word 1.1.
%Copyright (C) 1992-93 TCI Software Research, Inc.
\typeout{TCILCOMM Macros for TCI styles <08 Apr 93>.}
%
% Revisions:
% 08 Apr 93 - GP change line length to under 80 characters
% 30 Mar 92 - AO added \setmoremathsizes and hooks to, e.g. \@xpt,
%             for support of bold Greek
%
%%ltg added this to try to get 12pt to come through
%\DeclareOption{12pt}{\renewcommand\@ptsize{2}}
%%end ltg

\def\@ptoptions{%
 \let\@elt\relax\@for\@tempa:=\@optionlist\do{%
  \expandafter\let\expandafter\@tempb\csname ds@\@tempa\endcsname
  \expandafter\let\expandafter\@tempc\csname ds@11pt\endcsname
  \ifx\@tempb\@tempc\else
   \expandafter\let\expandafter\@tempc\csname ds@12pt\endcsname
   \ifx\@tempb\@tempc\else\let\@tempb\relax\fi
   \fi
  \@tempb
  }%
 }%
%
% read in style file, but only process the pt size options
%
\def\@ptoptinput#1{%
 \let\@save@optionlist\@optionlist
 \let\@save@options\@options
 \let\@options\@ptoptions
 %
 \input #1
 %
 \let\@optionlist\@save@optionlist
 \let\@options\@save@options
 }%
%
% the <21 Feb 92> version of letter.sty requires:
\ifx\undefined\reset@font
 \def\reset@font{}%
 \fi
%
% Change LaTeX
%
% Add command to append tokens
\newtoks\@temptokenb
\long\def\appdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokena\the\@temptokenb}%
 }%
\long\def\prepdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokenb\the\@temptokena}%
 }%
% Discard contents of \box\@cclv at beginning of document
\appdef\document{{\output{\setbox\z@\box\@cclv}\endgraf\null\eject}}%
% Fix mark register expansion
\def\leftmark{\expandafter\@leftmark\botmark{}{}{}\@nil}%
\def\rightmark{\expandafter\@rightmark\firstmark{}{}{}\@nil}%
\def\@leftmark#1#2#3\@nil{#1}%
\def\@rightmark#1#2#3\@nil{#2}%
%
%\show\raggedright
\newskip\raggedglue
\raggedglue\z@ plus20\p@ minus\z@
\def\raggedright{%
 \let\\=\@centercr\@rightskip\raggedglue\rightskip
 \@rightskip\leftskip\z@\parindent\z@
 }%
%
\def\@centercr{%
 \ifhmode\unskip\else\@badcrerr\fi\@@par
 \@ifstar{\penalty\@M\@xcentercr}{\@xcentercr}%
 }%
%
\def\traceoutput{\tracingoutput2\showboxbreadth\maxdimen
 \showboxdepth\maxdimen}%
%
\newcount\@hour\newcount\@minute\chardef\@x10\chardef\@xv60
\def\@time{%
  \@minute\time\@hour\@minute\divide\@hour\@xv
  \ifnum\@hour<\@x 0\fi\the\@hour:%
  \multiply\@hour\@xv\advance\@minute-\@hour
  \ifnum\@minute<\@x 0\fi\the\@minute
  }%
%
% change \@array to allow \par to mean something within its scope
%
\def\@array [#1]#2{%
 \setbox\@arstrutbox\hbox{\vrule height\arraystretch\ht
  \strutbox depth\arraystretch\dp\strutbox width\z@}%
 \@mkpream{#2}%
 \edef\@preamble{\halign\noexpand\@halignto\bgroup\tabskip
  \z@\@arstrut\@preamble\tabskip\z@\cr}%
 \let\@startpbox\@@startpbox\let\@endpbox\@@endpbox
 \if#1t\vtop\else\if#1b\vbox\else\vcenter\fi\fi
 \bgroup
  %\let\par\relax
  \let\@sharp##
  \let\protect\relax
  \lineskip\z@\baselineskip\z@
  \@preamble
 }%
%
% Expands to hex digit corresponding to the value of the argument
%
\def\hexnumber@#1{\ifnum#1<10 \number#1\else
 \ifnum#1=10 A\else\ifnum#1=11 B\else\ifnum#1=12 C\else
 \ifnum#1=13 D\else\ifnum#1=14 E\else\ifnum#1=15 F\fi\fi\fi\fi\fi\fi\fi}%
%
% define command to set more math sizes.
% Styles like Greekbf will hook in here.
%
\def\setmoremathsizes#1#2#3{}%
%
% define size switch addenda
%  Note: these choices agree with those in lfonts.tex, even if incorrect.
%
\prepdef\@vpt{\setmoremathsizes{fiv}{fiv}{fiv}}%
\prepdef\@vipt{\setmoremathsizes{six}{six}{six}}%
\prepdef\@viipt{\setmoremathsizes{sev}{fiv}{fiv}}%
\prepdef\@viiipt{\setmoremathsizes{egt}{six}{fiv}}%
\prepdef\@ixpt{\setmoremathsizes{nin}{six}{fiv}}%
\prepdef\@xpt{\setmoremathsizes{ten}{sev}{fiv}}%
\prepdef\@xipt{\setmoremathsizes{elv}{egt}{six}}%
\prepdef\@xiipt{\setmoremathsizes{twl}{egt}{six}}%
\prepdef\@xivpt{\setmoremathsizes{frtn}{ten}{sev}}%
\prepdef\@xviipt{\setmoremathsizes{svtn}{twl}{ten}}%
\prepdef\@xxpt{\setmoremathsizes{twty}{frtn}{twl}}%
\prepdef\@xxvpt{\setmoremathsizes{twty}{twty}{svtn}}%
%
% The \newfield command defines (like \newenvironment) a user syntax:
%
%   \newfield{foo}
%
% lets you write
%
%   \begin{foo}...\end{foo}
%
% but differs from \newenvironment in that TeX parses the entire content
% of the field and stores it in a macro \the@foo, and then executes \@do@foo.
%
% This means that the content of the field is actually more like an argument
% than the content of an environment. So \verb will not necessarily work
% within a field, and neither will \index. Caveat emptor.
%
% The default procedure for a field is to process its argument within a
% group.  If you want a field to simply store its data away, define its
% procedure to be synonymous with \@empty, as illustrated below.
%
\long\def\@readenvir#1#2\end{%
 \appdef\envirsofar{#2}%
 \@ifnextchar\bgroup{\@checkenvir{#1}}{\@envirenderr}%
 }%
%
\def\@envirenderr{%
 \@latexerr{\string\end\space not followed by environment name}\@eha
 }%
%
\def\@checkenvir#1#2{%
 \def\@tempa{#1}\def\@tempb{#2}%
 \ifx\@tempa\@tempb
  \ifx\envirsofar\@blankspace\let\envirsofar\@empty\fi
  \expandafter\let\csname the@#1\endcsname\envirsofar
  \def\@tempa{\csname @do@#1\endcsname}%
  \else
  \appdef\envirsofar{\end{#2}}%
  \def\@tempa{\@readenvir{#1}}%
  \fi
 \@tempa
 }%
%
\def\newfield#1#2{%
 \expandafter\@ifdefinable\csname#1\endcsname{%
  \expandafter\def\csname#1\endcsname{%
   \endgroup\let\envirsofar\@empty\@readenvir{#1}%
   }%
  \expandafter\let\csname the@#1\endcsname\@empty
  \expandafter\ifx\csname @do@#1\endcsname\relax
   \expandafter\def\csname @do@#1\endcsname{{\csname the@#1\endcsname}}%
   \fi
  }%
 }%
%
\def\@blankspace{ }% SciWord's nil field
%
\def\letparBL{\def\par{\\}}%
\def\letparSP{\def\par{\ }}%
\def\letparQD{\def\par{\quad}}%
\def\letparSL{\def\par{\hbox to1em{\hfil/\hfil}}}%
%
% When \par is processed in the page head, gobble up the rest of the
% argument.
\def\@gobblepar#1\@empty{}%
%
% Physical page size after trim
\newdimen\trimwidth
\newdimen\trimheight
\newdimen\botmargin
\newdimen\marginpartotal
%
\def\adjustpagemargin{% adjust \oddsidemargin by \marginpartotal
 \marginpartotal\marginparwidth\advance\marginpartotal\marginparsep
 \advance\oddsidemargin\marginpartotal
 }%
%
\def\settextheight{% calculate textheight constrained by:
 \textheight\trimheight
 \advance\textheight-\topmargin
 \advance\textheight-\headheight
 \advance\textheight-\headsep
 \advance\textheight-\footskip
 \advance\textheight-\botmargin
 }%
%
\def\vcenterpagemargin{% calculate \topmargin constrained by:
 \topmargin\trimheight
 \advance\topmargin-\textheight
 \advance\topmargin-\headheight
 \advance\topmargin-\headsep
 \advance\topmargin-\footskip
 \divide\topmargin\tw@\botmargin\topmargin
 }%
%
\def\centerpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \divide\oddsidemargin\tw@
 \evensidemargin\oddsidemargin
 \adjustpagemargin
 }%
%
\def\leftpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \advance\oddsidemargin-\evensidemargin
 \adjustpagemargin
 }%

